The workweek is the best time to start a family -- A Study of GPT-2 Based Claim Generation

Argument generation is a challenging task whose research is timely considering its potential impact on social media and the dissemination of information. Here we suggest a pipeline based on GPT-2 for generating coherent claims, and explore the types of claims that it produces, and their veracity, using an array of manual and automatic assessments. In addition, we explore the interplay between this task and the task of Claim Retrieval, showing how they can complement one another.

==> dev_topics.tex <==
\begin{table}[h]
\begin{center}
\scriptsize
\begin{tabular}{|p{7cm}|}
\hline
We should legalize doping in sport                               \\ \hline
We should protect endangered species                             \\ \hline
We should legalize insider trading                               \\ \hline
We should lower the drinking age                                 \\ \hline
We should abolish temporary employment                           \\ \hline
We should ban free newspapers                                    \\ \hline
We should abolish the US Electoral College                       \\ \hline
We should ban lotteries                                          \\ \hline
We should legalize ivory trade                                   \\ \hline
We should further exploit green technology                       \\ \hline
We should ban abortions                                          \\ \hline
We should further exploit geothermal energy                      \\ \hline
We should raise the retirement age                               \\ \hline
We should ban alternative medicine                               \\ \hline
We should subsidize public service broadcasters                  \\ \hline
We should abolish term limits                                    \\ \hline
We should abandon Gmail                                          \\ \hline
We should not subsidize single parents                           \\ \hline
We should introduce school vouchers                              \\ \hline
Prenatal diagnosis should be mandatory                           \\ \hline
We should prohibit tower blocks                                  \\ \hline
We should increase airport racial profiling in the United States \\ \hline
We should increase international volunteering                    \\ \hline
We should subsidize the human mission to Mars                    \\ \hline
The use of AI should be abandoned                                \\ \hline
We should fight for Palestinian independence                     \\ \hline
We should further exploit natural gas                            \\ \hline
We should abandon democracy                                      \\ \hline
We should ban fishing                                            \\ \hline
We should ban gratuities                                         \\ \hline
We should increase government regulation                         \\ \hline
Community service should be mandatory                            \\ \hline
We should further exploit solar energy                           \\ \hline
Tattoos should be banned                                         \\ \hline
We should support a phase-out of lightweight plastic bags       \\ \hline
\end{tabular}
\end{center}
\caption{List of dev set topics.}
\end{table}

==> test_topics.tex <==
\begin{table}[t]
\begin{center}
\scriptsize
\begin{tabular}{|p{7cm}|}
\hline
We should end the use of solitary confinement         \\ \hline
We should disband the United Nations Security Council \\ \hline
We should end the use of mass surveillance            \\ \hline
Child labor should be legalized                       \\ \hline
We should cancel the pledge of allegiance to the flag \\ \hline
We should ban multi-level marketing                   \\ \hline
We should adopt environmental justice                 \\ \hline
We should ban media conglomerates                     \\ \hline
We should end the use of traffic enforcement cameras  \\ \hline
We should introduce a national identity card          \\ \hline
We should subsidize transportation network companies  \\ \hline
We should ban burqas                                  \\ \hline
We should ban conversion therapy                      \\ \hline
We should introduce the alternative vote              \\ \hline
Force-feeding should be banned                        \\ \hline
We should abandon tabloid journalism                  \\ \hline
We should legalize LGBT adoption                      \\ \hline
We should abandon Twitter                             \\ \hline
We should abandon chain stores                        \\ \hline
We should further exploit mixed-use development       \\ \hline
We should subsidize open access journals              \\ \hline
We should end child benefits                          \\ \hline
We should increase the use of telemedicine            \\ \hline
We should abandon the sexual revolution               \\ \hline
We should adopt polyamory                             \\ \hline
We should end the use of bailouts                     \\ \hline
Begging should be banned                              \\ \hline
We should adopt catholicism                           \\ \hline
We should abolish credit scores                       \\ \hline
We should fight environmental degradation             \\ \hline
We should increase environmental protection           \\ \hline
Flu vaccination should be mandatory                   \\ \hline
We should close landfills                             \\ \hline
We should further exploit filibusters                 \\ \hline
Minority groups should be protected                   \\ \hline

% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[t]
% \begin{center}
% \scriptsize
% \begin{tabular}{|p{7cm}|}
% \hline

We should limit the use of petroleum                  \\ \hline
We should end privatization                           \\ \hline
We should increase the use of probation               \\ \hline
We should increase the use of rapid transit           \\ \hline
We should increase the use of scholarships            \\ \hline
We should abandon weddings                            \\ \hline
We should ban Gerrymandering                          \\ \hline
We should increase the use of background checks       \\ \hline
We should ban billboards                              \\ \hline
We should limit campaign finance                      \\ \hline
We should abolish competition laws                    \\ \hline
We should subsidize financial advisors                \\ \hline
We should protect freedom of religion                 \\ \hline
We should introduce guaranteed minimum income         \\ \hline
We should limit judicial review                       \\ \hline
We should subsidize medical schools                   \\ \hline
We should ban the use of migrant workers              \\ \hline
We should abolish dual citizenship                    \\ \hline
We should abolish the presidential pardon             \\ \hline
We should increase the use of part-time contracts     \\ \hline
We should abandon the presidential system             \\ \hline
We should end the use of public housing               \\ \hline
We should limit the use of appeals                    \\ \hline
We should protect animal welfare                      \\ \hline
We should increase consumer protection                \\ \hline
We should abolish emissions trading                   \\ \hline
We should disband the G20                             \\ \hline
We should fight sedentary lifestyle                   \\ \hline
We should prohibit over the counter drugs             \\ \hline
We should increase the use of public spaces           \\ \hline
We should abandon Valentine's day                     \\ \hline
We should abandon voter registration                  \\ \hline
We should increase the workweek                       \\ \hline
We should prohibit carrying a concealed weapon        \\ \hline
We should abandon Zionism                             \\ \hline
We should further exploit genetic engineering         \\ \hline
We should abandon brick and mortar companies          \\ \hline
We should limit Hydrocarbon exploration               \\ \hline

\end{tabular}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\scriptsize
\begin{tabular}{|p{7cm}|}
\hline

We should nationalize the health care industry        \\ \hline
We should increase trade barriers                     \\ \hline
We should fight the gender pay gap                    \\ \hline
We should subsidize Anti-diabetic medication          \\ \hline
We should fight illegal logging                       \\ \hline
We should ban rodenticide                             \\ \hline
We should ban chewing tobacco                         \\ \hline
We should further exploit enhanced oil recovery       \\ \hline
The Euro should be abandoned                          \\ \hline
We should ban alcohol advertising                     \\ \hline
Blood donation should be mandatory                    \\ \hline
We should abandon motorcycles                         \\ \hline
We should increase the use of artificial insemination \\ \hline
Emergency contraception should be subsidized          \\ \hline
We should abandon speed limit enforcement             \\ \hline
Criticism of the Iraq War is justified                \\ \hline
We should disband Planned Parenthood                  \\ \hline
We should prohibit subprime lending                   \\ \hline
We should abandon alimony                             \\ \hline
We should ban attack ads                              \\ \hline
Jury duty should not be mandatory                     \\ \hline
We should subsidize adult learners                    \\ \hline
We should not abandon the Paris Agreement             \\ \hline
\end{tabular}
\end{center}
\caption{List of test set topics.}
\end{table}
